Physics-Guided Adversarial Machine Learning for Aircraft Systems Simulation

In the context of aircraft system performance assessment, deep learning technologies allow to quickly infer models from experimental measurements, with less detailed system knowledge than usually required by physics-based modeling. However, this inexpensive model development also comes with new challenges regarding model trustworthiness. This work presents a novel approach, physics-guided adversarial machine learning (ML), that improves the confidence over the physics consistency of the model. The approach performs, first, a physics-guided adversarial testing phase to search for test inputs revealing behavioral system inconsistencies, while still falling within the range of foreseeable operational conditions. Then, it proceeds with physics-informed adversarial training to teach the model the system-related physics domain foreknowledge through iteratively reducing the unwanted output deviations on the previously-uncovered counterexamples. Empirical evaluation on two aircraft system performance models shows the effectiveness of our adversarial ML approach in exposing physical inconsistencies of both models and in improving their propensity to be consistent with physics domain knowledge.

==> tables2/RQ1.tex <==
\begin{table}[ht]
\centering
\caption{The number of unique exposed adversarial cases on train and test datasets per search method and system}
\label{tab:RQ1}
\begin{tabular}{|l|l|l|l|l|}
\hline     
\textbf{SYS}        & \textbf{Method}         & \textbf{G} & \textbf{Dataset} & \textbf{Avg. \#AdvIn} \\ \hline
\multirow{12}{*}{A-C Perf.} & \multirow{4}{*}{RS} & 361K   & $D_{train}$& 1302.3 \\ \cline{4-5}                            &                         & 40K   & $D_{test}$& 128.1 \\ \cline{3-5} 
                       &                         & 903K   & $D_{train}$& 3186.4 \\ \cline{3-5}                            &              & 100K    & $D_{test}$& 340.3 \\ \cline{2-5} 
                       & \multirow{4}{*}{PSO}    & 361K   & $D_{train}$& 9340.3 \\ \cline{3-5}                            &                         & 40K    & $D_{test}$& 1127.4 \\ \cline{3-5}  
                       &                         & 903K   & $D_{train}$& 25134.4 \\ \cline{3-5}                            &                         &   100K  & $D_{test}$& 2827.7 \\ \cline{2-5} 
                       & \multirow{4}{*}{GA}    & 361K   & $D_{train}$& 919.7 \\ \cline{3-5}                            &                         &  40K   & $D_{test}$& 75.6 \\ \cline{3-5} 
                       &                         & 903K   & $D_{train}$& 2161.0 \\ \cline{3-5}                            &                         &  100K   & $D_{test}$& 209.4\\ \hline 
\multirow{12}{*}{WAI Perf.} & \multirow{4}{*}{RS} & 361K   & $D_{train}$& 29.5 \\ \cline{4-5}                            &                         &   40K & $D_{test}$& 3.3 \\ \cline{3-5} 
                       &                         & 903K   & $D_{train}$& 67.2 \\ \cline{3-5}                            &                         &  100K   & $D_{test}$& 9.4 \\ \cline{2-5} 
                       & \multirow{4}{*}{PSO} & 361K   & $D_{train}$& 1099.8 \\ \cline{3-5}                            &                         &  40K   & $D_{test}$& 113.2 \\ \cline{3-5} 
                       &                         & 903K   & $D_{train}$& 3884.6 \\ \cline{3-5}                            &           &  100K   & $D_{test}$& 400.4 \\ \cline{2-5} 
                       & \multirow{4}{*}{GA}    & 361K   & $D_{train}$& 17.0 \\ \cline{3-5}                            &                         &   40K  & $D_{test}$& 1.2 \\ \cline{3-5} 
                       &                         & 903K   & $D_{train}$& 56.1 \\ \cline{3-5}                            &                         &  100K   & $D_{test}$& 12.1 \\ \hline 
\end{tabular}
\end{table}                         

==> tables2/RQ2.tex <==
\begin{table}[ht]
\centering
\caption{Average ratio of valid test inputs and duplicated adversarial examples per SBST algorithm and per system}
\label{tab:RQ2}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{SYS} & \textbf{ALG} & \textbf{Avg. \%ValIn} & \textbf{Avg. \%DupIn}\\ \hline
\multirow{3}{*}{A-C Perf.}   & RS  & 31.40\%  & 0\%  \\ \cline{2-4} 
                       & PSO  & 44.35\%  & 31.61\% \\ \cline{2-4} 
                       & GA & 27.55\% &  10.47\% \\ \hline
\multirow{3}{*}{WAI Perf.} & RS  & 90.16\% & 0\% \\ \cline{2-4} 
                       & PSO  & 99.12\% & 81.56\%  \\ \cline{2-4} 
                       & GA & 82.45\% & 34.84\%  \\ \hline
\end{tabular}
\end{table}

==> tables2/RQ3.tex <==
\begin{table}[ht]
\centering
\caption{comparison between \#adversarials before and after fine-tuning fix}
\label{tab:RQ3}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{SYS} & \textbf{G} & \textbf{pre-\#AdvIn} & \textbf{post-\#AdvIn} & \textbf{\%Improv\_AdvIn} \\ 
\hline
\multirow{3}{*}{A-C Perf.}   & RS  & 5267  & 1012   & 80.78\% \\ \cline{2-5} 
                             & PSO  & 39551  & 5747	  & 85.46\%        \\ \cline{2-5} 
                             & GA & 2850 & 636  & 77.68\%        \\ \hline
\multirow{3}{*}{WAI Perf.}   & RS  & 509  & 0   & 100\% \\ \cline{2-5} 
                       & PSO  & 20545	 & 18   &  99.91\%       \\ \cline{2-5} 
                       & GA &  459  & 4   &  99.12\%       \\ \hline
\end{tabular}
\end{table}

==> tables2/RQ4.tex <==
\begin{table}[ht]
\centering
\caption{Comparison between RMSE after and before fine-tuning fix}
\label{tab:RQ4}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{SYS} & \textbf{TRG}   & \textbf{pre-RMSE}  & \textbf{ALG} & \textbf{post-RMSE} & \shortstack{\textbf{\%Chg} \\ \textbf{RMSE}}\\\hline
\multirow{3}{*}{A-C Perf.}   
& \multirow{3}{*}{$\alpha$} 
& \multirow{3}{*}{0.498°}  
& RS& 0.497°& \textcolor{dkgreen}{-0.20}\\ \cline{4-6} 
&  &  & PSO & 0.996°& \textcolor{red}{+100}\\ \cline{4-6} 
&  &  & GA& 0.444°& \textcolor{dkgreen}{-10.84}\\ \hline
\multirow{6}{*}{WAI Perf.} & 
\multirow{3}{*}{$T_{skin}^a$}& 
\multirow{3}{*}{4.088°C} 
& RS & 4.729°C& \textcolor{red}{+15.68}\\ \cline{4-6} 
&  &  & PSO & 4.422°C& \textcolor{red}{+8.17}\\ \cline{4-6} 
&  &  & GA & 3.979°C& \textcolor{dkgreen}{-2.67}\\ \cline{2-6} 
& \multirow{3}{*}{$T_{skin}^b$} & 
\multirow{3}{*}{7.524°C} 
& RS & 7.921°C& \textcolor{red}{+5.28}\\ \cline{4-6} 
&  &  & PSO& 6.826°C& \textcolor{dkgreen}{-9.28}\\ \cline{4-6} 
&  &  & GA& 7.163°C& \textcolor{dkgreen}{-4.80}\\ \hline
\end{tabular}
\end{table}

==> tables2/ac_perf_rules.tex <==
\begin{table}[h]
\centering
\caption{Physics-grounded Sensitivity Rules for A/C Perf. Model}
\label{tab:AOA_rules}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Rule}  & \textbf{Premises}    & \textbf{Conclusion}  \\ \hline
$r_0\in R_{incr}$ & CAS $\downarrow$ , ACWT $\uparrow$ , Flap $\downarrow$ , Slat $\downarrow$ & $\alpha$ $\uparrow$ \\ \hline
$r_1\in R_{decr}$ & CAS $\uparrow$, ACWT $\downarrow$, Flap $\uparrow$, Slat$\uparrow$ & $\alpha\downarrow$ \\ \hline
$r_2\in R_{cons}$ & CAS $\leftrightarrow$ , ACWT $\leftrightarrow$ & $\alpha$ $\leftrightarrow$ \\ \hline
\end{tabular}
\end{table}

==> tables2/table_2.tex <==
\begin{table}[h]
\centering
\caption{Aircraft performance Data Catalog}
\label{tab:AOA-reg-data-catalog}
%\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|l|}
\cline{2-3}
& \textbf{Name}  & \textbf{Type}  \\ 
\hline
\multicolumn{1}{|l|}{
\multirow{4}{*}{\textbf{Features}}} & Calibrated Airspeed& Real\\ 
\cline{2-3} 
\multicolumn{1}{|l|}{} & Aircraft Weight& Real\\ 
\cline{2-3} 
\multicolumn{1}{|l|}{} & Slat Angle& Dichotomous\\ 
\cline{2-3} 
\multicolumn{1}{|l|}{} & Flap Angle& Categorial\\
\hline
\multicolumn{1}{|l|}{\textbf{Target}} & Angle of Attack& Real\\ 
\hline
\end{tabular}
%}
\end{table}

==> tables2/table_3.tex <==
\begin{table}[h]
\centering
\caption{WAI Performance Data Catalog}
\label{tab:WAIS-temp-reg-data-catalog}
\begin{tabular}{l|l|l|}
\cline{2-3}
& \textbf{Name}& \textbf{Type} \\ \hline
\multicolumn{1}{|l|}{\multirow{8}{*}{\textbf{Features}}} & Angle of Attack & Real\\ \cline{2-3} 
\multicolumn{1}{|l|}{}                                   & True Airspeed& Real\\ \cline{2-3} 
\multicolumn{1}{|l|}{}                                   & Pressure Altitude& Real\\ \cline{2-3} 
\multicolumn{1}{|l|}{}                                   & Pressure of Wing Root& Real\\ \cline{2-3} 
\multicolumn{1}{|l|}{}                                   & Temperature of Wing Root& Real\\ \cline{2-3} 
\multicolumn{1}{|l|}{}                                   & Total Air Temperature& Real\\ \cline{2-3} 
\multicolumn{1}{|l|}{}                                   & Slat Angle & Dichotomous \\ \cline{2-3} 
\multicolumn{1}{|l|}{}                                   & Flap Angle& Categorical\\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Target}}} & 
A-Wing's Skin Temperature Sensor & Real \\ 
\cline{2-3} 
\multicolumn{1}{|l|}{}&  B-Wing's Skin Temperature Sensor & Real \\ 
\hline
\end{tabular}
\end{table}

==> tables2/wais_aug_rules.tex <==
\begin{table}[h]
\renewcommand{\arraystretch}{1.5}
\centering
\caption{Augmentation Rules for WAIS Perf. Model}
\label{tab:Aug_WAIS_rules}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Status} & \textbf{Rule} & \textbf{Premises} & \textbf{Conclusion} \\ \hline
\multirow{3}{*}{ON}&\multirow{2}{*}{$A_1$} & TAT $+$ $t$ , TWR $+$ $t$ , & 
\multirow{2}{*}{$T_{skin}^{a,b}$ $+$ $t$} \\ %\cline{3-4} 
&&$\forall t\in[-10, 10]$ & \\ \cline{2-4} 
&$A_2$ & PWR $= 0$ & $T_{skin}^{a,b}$ $=$ TAT \\ \cline{2-4} 
&$A_3$ & TAS $= 0$ & $T_{skin}^{a,b}$ $=$ TWR \\ \hline
OFF& $A_3$ & TWR $=$ TAT & $T_{skin}^{a,b}$ $=$ TAT\\ \hline
\end{tabular}
\end{table}


==> tables2/wais_perf_rules.tex <==
\begin{table}[h]
\renewcommand{\arraystretch}{1.5}
\centering
\caption{Physics-grounded Sensitivity Rules for WAIS Perf. Model}
\label{tab:WAIS_rules}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Status} & \textbf{Rule} & \textbf{Premises} & \textbf{Conclusion} \\ \hline
\multirow{2}{*}{ON}      & \multirow{2}{*}{$r_3\in R_{incr}$ } & ALT $\uparrow$ , TWR $\uparrow$ , PWR $\uparrow$ , & \multirow{2}{*}{$T_{skin}^{a,b}$ $\uparrow$} \\ 
&&TAT $\uparrow$ , TAS $\downarrow$ , $\alpha$ $\downarrow$ &  \\ \cline{2-4} 
                             & \multirow{2}{*}{$r_4\in R_{decr}$} & ALT $\downarrow$ , TWR $\downarrow$ , PWR $\downarrow$ , & \multirow{2}{*}{$T_{skin}^{a,b}$ $\downarrow$} \\ 
                          && TAT $\downarrow$ , TAS $\uparrow$ , $\alpha$ $\uparrow$ & \\ \hline
\multirow{2}{*}{OFF}   & $r_5\in R_{incr}$  & TAT $\uparrow$ , PWR $\uparrow$ , $\alpha$ $\downarrow$  & $T_{skin}^{a,b}$ $\uparrow$  \\ \cline{2-4} 
                           & $r_6\in R_{decr}$ &  TAT $\downarrow$ , PWR $\downarrow$ , $\alpha$ $\uparrow$  & $T_{skin}^{a,b}$ $\downarrow$     \\ \hline
\multirow{2}{*}{Both} & \multirow{2}{*}{$r_7\in R_{cons}$} &  ALT $\leftrightarrow$ , TWR $\leftrightarrow$ , PWR $\leftrightarrow$ , & \multirow{2}{*}{$T_{skin}^{a,b}$ $\leftrightarrow$} \\
&& TAT $\leftrightarrow$ , TAS $\leftrightarrow$ , $\alpha$ $\leftrightarrow$&\\ \hline
\end{tabular}
\end{table}
